SemEval-2016 Task 3: Community Question Answering

This paper describes the SemEval--2016 Task 3 on Community Question Answering, which we offered in English and Arabic. For English, we had three subtasks: Question--Comment Similarity (subtask A), Question--Question Similarity (B), and Question--External Comment Similarity (C). For Arabic, we had another subtask: Rerank the correct answers for a new question (D). Eighteen teams participated in the task, submitting a total of 95 runs (38 primary and 57 contrastive) for the four subtasks. A variety of approaches and features were used by the participating systems to address the different subtasks, which are summarized in this paper. The best systems achieved an official score (MAP) of 79.19, 76.70, 55.41, and 45.83 in subtasks A, B, C, and D, respectively. These scores are significantly better than those for the baselines that we provided. For subtask A, the best system improved over the 2015 winner by 3 points absolute in terms of Accuracy.

==> discussion.tex <==
% !TEX root = main.tex
%%% Section 7: Discussion

- Combine the top-n systems -- ensemble

- Stat. significance

- Comparing outputs

- What examples everybody gets wrong/right

- smarter baselines: n-gram only

- are people using semantic/syntactic info

- task C -- who is doing it really?

